Superconducting states of pure and doped graphene

We study the superconducting phases of the two-dimensional honeycomb lattice of graphene. We find two spin singlet pairing states, s-wave and an exotic $p+ip$ that is possible because of the special structure of the honeycomb lattice. At half filling, the $p+ip$ phase is gapless and superconductivity is a hidden order. We discuss the possibility of a superconducting state in metal coated graphene.

==> generated_files/paperID.tex <==


       *** SAVE THIS MESSAGE FOR FUTURE REFERENCE ***
          (and forward to any collaborators for safekeeping)

Your user/password combination for this paper is

 User-ID: cond-mat/0608515
 Password: k9bsq

You will need this ID/password pair to do any of the following:

  - to check the paper before it is announced
  - to cross-list the paper 
  - to add publication information
  - to replace the paper with a revised version

Keep this password safe -- all future replacements will require it.

Paper: cond-mat/0608515
From: Bruno Barboza Uchoa <uchoa@buphy.bu.edu>

Title: Superconductivity in metal coated graphene
Authors: B. Uchoa, and A. H. Castro Neto
Comments: 8 pages, 6 figures
Subj-class: Superconductivity; Materials Science id: 
